The qudit Pauli group: non-commuting pairs, non-commuting sets, and structure theorems

Qudits with local dimension $d>2$ can have unique structure and uses that qubits ($d=2$) cannot. Qudit Pauli operators provide a very useful basis of the space of qudit states and operators. We study the structure of the qudit Pauli group for any, including composite, $d$ in several ways. To cover composite values of $d$, we work with modules over commutative rings, which generalize the notion of vector spaces over fields. For any specified set of commutation relations, we construct a set of qudit Paulis satisfying those relations. We also study the maximum size of sets of Paulis that mutually non-commute and sets that non-commute in pairs. Finally, we give methods to find near minimal generating sets of Pauli subgroups, calculate the sizes of Pauli subgroups, and find bases of logical operators for qudit stabilizer codes. Useful tools in this study are normal forms from linear algebra over commutative rings, including the Smith normal form, alternating Smith normal form, and Howell normal form of matrices. Possible applications of this work include the construction and analysis of qudit stabilizer codes, entanglement assisted codes, parafermion codes, and fermionic Hamiltonian simulation.

==> noncommuting-sets-1qudit.tex <==
\section{Non-commuting sets of Paulis on 1 qudit}

On 1 qudit, Eq.~\eqref{eq:commutator} simplifies to
\begin{equation}
\llbracket P(a,b),P(s,t)\rrbracket_d = -\det\left(\begin{array}{cc}a&b\\s&t\end{array}\right)\mod{d}.
\end{equation}
As a consequence, finding the largest set of non-commuting Paulis on 1 qudit is equivalent to finding a maximum clique $C_m$ in the graph $G=(V,E)$ with vertices $V=\mathbb{Z}_d\times\mathbb{Z}_d$ and edge $((a,b),(s,t))\in E$ if and only if $\det\left(\begin{smallmatrix}a&b\\s&t\end{smallmatrix}\right)\neq0\mod{d}$.

Let us define $W\subseteq V$, where $(a,b)\in W$ if and only if $\gcd(a,b,d)=1$ (In this section, we evaluate $\gcd$ over $\mathbb{Z}$ and define it to be positive to ensure that it is unique).

\begin{lemma}\label{lem:G_properties}
The graph $G=(V,E)$ has the following properties.
\begin{enumerate}[(a)]
\item If $C\subseteq V$ is a clique in $G$, then there is a clique $C'\subseteq W$ of the same size, $|C|=|C'|$.  
\item If $v_0,v_2\in V$, $v_1\in W$, $(v_0,v_1)\not\in E$, and $(v_1,v_2)\not\in E$, then $(v_0, 
v_2)\not\in E$.
\item If $(a,b)$ and $(s,t)$ are in $W$, then $((a,b),(s,t))\not\in E$ if and only if there exists $u\in\mathbb{Z}$ with $\gcd(u,d)=1$ such that $(a,b)=u(s,t)$.
\end{enumerate}
\end{lemma}
\begin{proof}
To prove (a), we show that if $C\subseteq V$ is a clique, then for any $v=(a,b)\in C$, $C'=(C\setminus\{v\})\cup\{v'\}$, where $v'=v/\gcd(a,b,d)\in W$, is also a clique. Suppose for contradiction, there is some $(s,t)\in C$ that is connected by an edge to $v$ but not to $v'$. Then, for $g=\gcd(a,b,d)$, we have $\det\left(\begin{smallmatrix}a/g&b/g\\s&t\end{smallmatrix}\right)=0$ which implies $\det\left(\begin{smallmatrix}a&b\\s&t\end{smallmatrix}\right)=0$, contradicting that $(s,t)$ is connected to $v$.

Let $v_i=(a_i,b_i)$ for $i=0,1,2$. To prove (b), note that by Bezout's identity, there are integers $x,y,z$ such that $xa_1+yb_1+zd=\gcd(a_1,b_1,d)=1$. Let
\begin{equation}
A=\left(\begin{array}{ccc}a_0&b_0&xa_0+yb_0+zd\\a_1&b_1&1\\a_2&b_2&xa_2+yb_2+zd\end{array}\right).
\end{equation}
Due to the last column being a linear combination of the first two and $(d,d,d)$, $\det(A)=0\mod{d}$. Also, for $c_i=xa_i+yb_i+zd$, the cofactor expansion says $0=\det(A)=c_0\det\left(\begin{smallmatrix}a_1&b_1\\a_2&b_2\end{smallmatrix}\right)-\det\left(\begin{smallmatrix}a_0&b_0\\a_2&b_2\end{smallmatrix}\right)+c_2\det\left(\begin{smallmatrix}a_0&b_0\\a_1&b_1\end{smallmatrix}\right)=-\det\left(\begin{smallmatrix}a_0&b_0\\a_2&b_2\end{smallmatrix}\right)\mod{d}$, proving $(v_0,v_2)\not\in E$.

The reverse direction of part (c) is a simple calculation. The forward direction is more involved. Apply the Smith normal form algorithm to obtain $A=\left(\begin{smallmatrix}a&b\\s&t\end{smallmatrix}\right)=S^{-1}BT$ for invertible matrices $S,T\in\mathbb{Z}_d^{2\times2}$ and diagonal $B\in\mathbb{Z}_d^{2\times2}$ with $B_{00}=\gcd(a,b,s,t)$ and $B_{11}=\det(A)/B_{00}$. Since $((a,b),(s,t))\not\in E$, we know $\det(A)=0\mod{d}$, and because we also have $\gcd(a,b,d)=1$, $B_{11}=0\mod{d}$. Rearrange to obtain $SA=BT$ and note that the last row of $BT$ is $(0,0)$. This implies 
\begin{equation}\label{eq:linear_combo}
S_{10}(a,b)+S_{11}(s,t)=(0,0).
\end{equation}
This equation means $\gcd(S_{10},d)$ divides $S_{11}s$ and $S_{11}t$. Because $\gcd(s,t,d)=1$, it must be that $\gcd(S_{10},d)$ divides $S_{11}$. Therefore, $\gcd(S_{10},d)$ divides $\det(S)$. Since $S$ is invertible, $\det(S)$ is a unit of the ring $\mathbb{Z}_d$, so its only divisors are other units. This means $\gcd(S_{10},d)=1$, and likewise, we can argue $\gcd(S_{11},d)=1$. So $S_{10}$, $S_{11}$, and $S_{11}/S_{10}$ are all units. Divide Eq.~\eqref{eq:linear_combo} by $S_{10}$ and rearrange to finish the proof.
\end{proof}

Lemma \ref{lem:G_properties}(a) implies there is a maximum clique that is just a subset of $W$. Part (b) implies transitivity of an equivalence relation $u\sim v$ for $u,v\in W$, where $u$ and $v$ are said to be equivalent if $(u,v)\not\in E$. Part (c) says equivalence classes of $W$ are all the same size, exactly the size of the group of units of $\mathbb{Z}_d$, which is $\phi(d)=d\prod_{p\mid d}(1-1/p)$, the Euler's totient function, where the product is over unique primes dividing $d$. Combining these facts, the size of a maximum clique of $G$ is $|C_m|=|W|/\phi(d)$.

To count $|W|$, we let $(a,b)\in W$ and allow $a\in\mathbb{Z}_d$ to be arbitrary. Now $b\in\mathbb{Z}_d$ is restricted by the choice of $a$. Namely, $b$ cannot share any prime factors with $\gcd(a,d)$. Each prime factor $p$ of $\gcd(a,d)$ reduces the allowable set of $b$ by a factor of $(p-1)/p=(1-1/p)$. We thus have
\begin{equation}
\frac1d|W|=\sum_{a\in\mathbb{Z}_d}\prod_{p\mid\gcd(a,d)}\left(1-\frac1p\right)\equiv F(d).
\end{equation}

It turns out $F$ is multiplicative.
\begin{lemma}
If $d_0,d_1\in\mathbb{Z}$ are relatively prime, then $F(d_0d_1)=F(d_0)F(d_1)$.
\end{lemma}
\begin{proof}
By Bezout's identity, there are integers $x_0,x_1$ such that $x_0d_0+x_1d_1=1$. Note that $x_0$ is an inverse of $d_0$ modulo $d_1$, so $\gcd(x_0,d_1)=1$. Likewise $\gcd(x_1,d_0)=1$. 

The Chinese remainder theorem implies there is an isomorphism between $\mathbb{Z}_{d_0d_1}$ and $\mathbb{Z}_{d_0}\times\mathbb{Z}_{d_1}$. Explicitly, it is $a= a_0\mod{d_0}$ and $a=a_1\mod{d_1}$, if and only if $a=a_0x_1d_1+a_1x_0d_0\mod{d_0d_1}$. This means that $\gcd(a,d_0)=\gcd(a_0,d_0)$ and $\gcd(a,d_1)=\gcd(a_1,d_1)$. We also have $\gcd(a,d_0d_1)=\gcd(a,d_0)\gcd(a,d_1)$.

Putting these facts together, we complete the proof:
\begin{align}
F(d_0d_1)&=\sum_{a\in\mathbb{Z}_{d_0d_1}}\prod_{p\mid\gcd(a,d_0d_1)}(1-1/p)\\&=\sum_{a_0\in\mathbb{Z}_{d_0}}\sum_{a_1\in\mathbb{Z}_{d_1}}\prod_{p|\gcd(a_0x_1d_1+a_1x_0d_0,d_0d_1)}(1-1/p)\\&=\sum_{a_0\in\mathbb{Z}_{d_0}}\prod_{p|\gcd(a_0,d_0)}(1-1/p)\sum_{a_1\in\mathbb{Z}_{d_1}}\prod_{p\mid\gcd(a_1,d_1)}(1-1/p)=F(d_0)F(d_1).
\end{align}
\end{proof}

It is easy to evaluate $F$ for prime powers: $F(p^k)=p^k(1-1/p^2)$. Consequently, $F(d)=d\prod_{p\mid d}(1-1/p^2)$ and
\begin{equation}
|C_m|=|W|/\phi(d)=dF(d)/\phi(d)=d\prod_{p\mid d}(1+1/p)=\Psi(d)
\end{equation}
which is sometimes referred to as the Dedekind $\Psi$ function.
